Dynamic Loop Fusion in High-Level Synthesis

Dynamic High-Level Synthesis (HLS) uses additional hardware to perform memory disambiguation at runtime, increasing loop throughput in irregular codes compared to static HLS. However, most irregular codes consist of multiple sibling loops, which currently have to be executed sequentially by all HLS tools. Static HLS performs loop fusion only on regular codes, while dynamic HLS relies on loops with dependencies to run to completion before the next loop starts. We present dynamic loop fusion for HLS, a compiler/hardware co-design approach that enables multiple loops to run in parallel, even if they contain unpredictable memory dependencies. Our only requirement is that memory addresses are monotonically non-decreasing in inner loops. We present a novel program-order schedule for HLS, inspired by polyhedral compilers, that together with our address monotonicity analysis enables dynamic memory disambiguation that does not require searching of address histories and sequential loop execution. Our evaluation shows an average speedup of 14$\times$ over static and 4$\times$ over dynamic HLS.

==> Figures/FigDeadlockWAW.tex <==
\begin{figure}[t]
\centering

    % \includegraphics[width=0.42\textwidth]{Figures/DeadlockWAW.pdf}
    % \caption{Code with a WAW hazard across loops (left) where all store addresses are equal to \texttt{10}. The corresponding LSUs (right) are in a state that will result in deadlock if \ref{eq:hazard} is used without modification.}


\begin{subfigure}[b]{0.45\textwidth}
\centering
\begin{verbatim}
for (i = 0; i<N; ++i)
    for (j = 0; j<M; ++j)
         // ..., {10, (1, 2)}, {10, (2, 3)}, ...
        store_b;
    for (k = 0; k<L; ++k)
        // {10, (1, 1)}, ...
        store_a;
\end{verbatim}
    \caption{Code with a WAW hazard across loops. The comments show $\{address, schedule\}$ for the stores.}
    \label{fig:DeadlockWAW_a}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.45\textwidth}
\centering
    \includegraphics[width=1\textwidth]{Figures/DeadlockWAW.pdf}
    \caption{The corresponding LSUs in a state that will result in deadlock if \ref{eq:hazard} is used without modification.}
\end{subfigure}

\caption{Repeated accesses to the same address might cause a deadlock if the \ref{eq:hazard} is not modified.}

\label{fig:DeadlockWAW}
\end{figure}


==> Figures/FigStoreLoadForwarding.tex <==
% \begin{figure}[t]
% \centering
% %  \begin{subfigure}[b]{0.45\textwidth}
% %  \centering
% %  \begin{verbatim}
% % for (i = 0; i < N; ++i)
% %   for (j = 0; j < M; ++j)
% %     // st addresses: 10, 11, 12, 13, 20, 21, 22, ..
% %     store A[f(i, j)];
% %   for (k = 0; k < L; ++k)
% %   // ld addresses: 21, ..
% %   load A[g(i, k)];
% % \end{verbatim}
% %      \caption{Code with a RAW hazard across loops with a potential for store-to-load forwarding.}
% %      \label{fig:StoreLoadForwarding_a}
% %  \end{subfigure}

%  % \begin{subfigure}[b]{0.45\textwidth}
%  %     \centering
%  %     \includegraphics[width=\textwidth]{Figures/StoreLoadForwarding_a.pdf}
%  %     \caption{Code with a RAW hazard across loops.}
%  %     \label{fig:StoreLoadForwarding_a}
%  % \end{subfigure}
%  % \hfill
%  % \begin{subfigure}[b]{0.45\textwidth}
%  %     \centering
%  %     \includegraphics[width=\textwidth]{Figures/StoreLoadForwarding_b.pdf}
%  %     \caption{LSU state with a possibility for store-to-load forwarding.}
%  %     \label{fig:StoreLoadForwarding_b}
%  % \end{subfigure}


% \includegraphics[width=0.42\textwidth]{Figures/StoreLoadForwarding.pdf}
% \caption{Code with a RAW hazard across loops (left) and the corresponding LSUs in a state that allows store-to-load forwarding (right).}

% \label{fig:StoreLoadForwarding}
% \end{figure}


\begin{figure}[t]
\centering


        % // {5, (1, 1)}, {10, (1, 2)}, 
        % // {15, (2, 3)}, .. 
% \begin{subfigure}[b]{0.45\textwidth}
% \centering
% \begin{verbatim}
% for (i = 0; i<N; ++i)
%     for (j = 0; j<2; ++j)
%         // .., {10, (1, 2)}, {15, (2, 3)}, .. 
%         store;
%     for (k = 0; k<2; ++k)
%         // {10, (1, 1)}, {11, (1, 2)}, ..
%         load;
% \end{verbatim}
%     \caption{Code with a RAW hazard across loops. The comments show the $\{address, schedule\}$ of the memory operation below.}
%     \label{fig:StoreLoadForwarding_a}
% \end{subfigure}
% \hfill
% \begin{subfigure}[b]{0.45\textwidth}
% \centering
%     \includegraphics[width=1\textwidth]{Figures/StoreLoadForwarding.pdf}
%     \caption{The corresponding DU state after two stores and zero loads.}
%     \label{fig:StoreLoadForwarding_b}
% \end{subfigure}

    \includegraphics[width=0.45\textwidth]{Figures/StoreLoadForwarding.pdf}
\caption{DU state that allows for store-to-load forwarding.}

\label{fig:StoreLoadForwarding}
\end{figure}

